Personalized Speech recognition on mobile devices

We describe a large vocabulary speech recognition system that is accurate, has low latency, and yet has a small enough memory and computational footprint to run faster than real-time on a Nexus 5 Android smartphone. We employ a quantized Long Short-Term Memory (LSTM) acoustic model trained with connectionist temporal classification (CTC) to directly predict phoneme targets, and further reduce its memory footprint using an SVD-based compression scheme. Additionally, we minimize our memory footprint by using a single language model for both dictation and voice command domains, constructed using Bayesian interpolation. Finally, in order to properly handle device-specific information, such as proper names and other context-dependent information, we inject vocabulary items into the decoder graph and bias the language model on-the-fly. Our system achieves 13.5% word error rate on an open-ended dictation task, running with a median speed that is seven times faster than real-time.

==> ep.tex <==
\section{Endpointer}
\label{sec:ep}

Our evaluations have thus far computed error rates without considering an important confounding variable in some domains: identifying end-of-speech.  When the recognizer automatically closes the microphone too early, this can directly impact word error rate.   We therefore adjust our evals to take endpointing into account and describe a smart endpointer that takes into account the end-of-sentence probability from the language model to decide when to close the microphone.

\begin{center}
\begin{tabular}{| l | l |}
\hline
LM Setup&Actions WER\\
\hline
GMM End-pointer~\cite{lei2013} & XX\\
\hline
Smart End-pointer & XX\\
\hline
\end{tabular}
\end{center}

% Decoder parameters (max\_arcs, etc)? Describe expanded search decoder algorithm?  Benchmark differences?


==> quantization.tex <==
\section{Quantization}
\label{sec:quantization}
Operating on a mobile device comes with significant computational constrains for the system. These constrains fall mainly in two categories:
\begin{enumerate}
  \item Memory consumption - driven by the need to make our application available in a variety of devices.
  \item Execution speed - out application must execute faster than real time to be usable.
\end{enumerate}

Since most of the memory and processing-time is consumed by the acoustic model neural network, we use quantization of the model's parameters (i.e. weights, biases) from their original floating point representation into a more compact 8-bit integer-based one. Being able to represent and operate on the parameters as small (8-bit) integers has an immediate impact in the memory usage. Moreover, in certain architectures, integer operations could be implemented more efficiently (e.g. NEON ARM SIMD can operate on eight 8-bit elements per instruction); additionally, smaller footprint matrices reduce data transfer when performing such operations, which is another cause of latency in mobile devices.

\subsection{Quantization basics}
\label{subsec:quantization_basics}
Quantizing means, in our case, mapping a set of values from a relatively high precision representation into a more constrained set of possible values. In this case let's consider the existing models' floating point parameters, and the desire to represent them as small 8-bit integer values.

Generally speaking we could use either a Uniform of a non-Uniform quantizer, or even an optimal quantizer for a given value distribution~\cite{bovik2005}. However, with simplicity and performance in mind, and validated by previous work in the area~\cite{vanhoucke2011}, we settled on a Uniform linear quantizer that assumes a uniform distribution of the values within a given range.

Thus, a simple mapping formula would find the original parameter values' range (i.e. min and max values), and then determine a scaling factor that when multiplied spreads those values evenly in the smaller precision scale, thus resulting in a quantized version of the originals.

\textbf{Quantizing.}
In the simple case of a set of float values $\mathbf{V}$, we perform the quantization of each value $V_{x}$ by computing a scaling factor $Q$ that when applied to the original $\mathbf{V}$ it will result in a approximated scaled $\mathbf{V'}$ that fits into the desired scale $S$ (e.g. 255 for 8-bits). To optimize the use of $S$ we determine the range of values $R = (V_\text{max} - V_\text{min})$ we want to quantize (i.e. squeeze into the new scale $S$). The quantization factor is then expressed as $Q = \frac{S}{R}$, and the quantization of a value as $V_{x}' = Q * (V_{x} - V_\text{min})$.

\textbf{Recovery.}
A quantized value $V_{x}'$ can be recovered (i.e. transformed back into its approximate original value) by performing the inverse quantization operation, which implies computing a recovery factor (the inverse of the quantization factor) $Q' = \frac{R}{S}$. The recovery of a value is then expressed as $V_{x} = V_{x}' * Q' + V_\text{min}$.


\textbf{Quantization error and bias}.
Quantization is a lossy process since it involves an approximation into a domain with less representational power than the original. As such, the quantization-recovery operations incur in an error which can be simply expressed as the difference between an input value and its quantized/recovered value. Something less obvious is that the quantization-recovery operations may incur in discrepancies that cause a bias in the computed value, and thus contribute to the quantization error.

From those two components of the quantization error, the precision-loss is theoretically and practically unavoidable and, on average, has a smaller impact on what the original data represents (such the difference on their variances is very small~\cite{gersho1992}). The bias however is theoretically avoidable by paying close attention at places where we manipulate quantized values, avoiding the introduction of inconsistencies. The latter is very important since bias problems have a big impact on the quantization error.


\subsection{Quantization implementation}
\label{subsec:quantization_implementation}
The approach we follow in our neural network inference is to operate in 8-bit integers everywhere except in the activation functions, and the final output of the network, which remain in floating point precision. Thus, from the operations performed for inference, multiplication (matrix dot product) is core, and has certain implications on how values are quantized and recovered.

\textbf{Multiplication of quantized values}.
Once we have quantized the network's parameters, and the inputs to the network, we perform operations on those values to carry the neural network inference. Thus, the multiplication of 2 independently quantized values $V_\text{a}'$ and $V_\text{b}'$, with quantization factors $Q_\text{a}$ and $Q_\text{b}$, produces a third value (the result) that’s being scaled by both $Q_\text{a}$ and $Q_\text{b}$. The other consideration is that in order to perform as much of the multiplication $V_\text{c} = V_\text{a} * V_\text{b}$ in the quantized domain, we must first apply the offset such that $V_\text{x} = \frac{V_\text{x}''}{Q}$, where  $V_\text{x}''=V_\text{x}' + Q V_\text{min}$. That way we perform most of the operation in 8-bit integers, applying the recovery factor on the result:

\begin{equation}
V_\text{c} = \frac{V_\text{a}'' * V_\text{b}''}{Q_\text{a} * Q_\text{b}}
\end{equation}


\textbf{Integer multiplication: effects on quantization and recovery}
The above multiplication, $V_\text{a}'' * V_\text{b}''$, performed in the quantized domain means that each factor $V_\text{x}''$ is of integer type. Such that in the $V_\text{x}''$ formulation: 1) $V_\text{x}'$ is already an integer; 2) $Q V_\text{min}$ is a float that will get round to an integer, and thus will introduce an error: $E = float(Q V_\text{min}) - integer(Q V_\text{min})$.

This means the quantization must be performed such that it is consistent with this formulation, or otherwise we would be introducing a bias. Thus we introduce a rounding operation $round()$:

\begin{equation}
V_\text{x}' = round(Q V_\text{x}) - round(Q V_\text{min})
\end{equation}

That way the precision errors in the quantization and multiplication are consistent and cancel each other.

This also means that recovery needs to operate in such way in order to be consistent with the quantization:

\begin{equation}
V_\text{x} = \frac{V_\text{x}' + round(Q V_\text{min})}{Q}
\end{equation}

\subsection{Quantization experiments}
\label{subsec:quantization_experiments}
Due to the loss of precision, quantization may have an impact on the accuracy of the inference, and thus the overal system's quality. Because of this, we are interested in finding ways of improving our quantization scheme, which due to its simplicity it meant exploring the impact of outliers in the neural network parameters that would affect our uniform-distribution assumption, blowing up the quantization range (thus reducing further the precision for the majority of the values).

